KET-QA: A Dataset for Knowledge Enhanced Table Question Answering

Due to the concise and structured nature of tables, the knowledge contained therein may be incomplete or missing, posing a significant challenge for table question answering (TableQA) and data analysis systems. Most existing datasets either fail to address the issue of external knowledge in TableQA or only utilize unstructured text as supplementary information for tables. In this paper, we propose to use a knowledge base (KB) as the external knowledge source for TableQA and construct a dataset KET-QA with fine-grained gold evidence annotation. Each table in the dataset corresponds to a sub-graph of the entire KB, and every question requires the integration of information from both the table and the sub-graph to be answered. To extract pertinent information from the vast knowledge sub-graph and apply it to TableQA, we design a retriever-reasoner structured pipeline model. Experimental results demonstrate that our model consistently achieves remarkable relative performance improvements ranging from 1.9 to 6.5 times and absolute improvements of 11.66% to 44.64% on EM scores across three distinct settings (fine-tuning, zero-shot, and few-shot), in comparison with solely relying on table information in the traditional TableQA manner. However, even the best model achieves a 60.23% EM score, which still lags behind the human-level performance, highlighting the challenging nature of KET-QA for the question-answering community. We also provide a human evaluation of error cases to analyze further the aspects in which the model can be improved. Project page: https://ketqa.github.io/.

==> tables/retriever_main_results_old.tex <==
\begin{table}[htbp]
\small % 调整表格字体大小
%\scriptsize
\begin{tabularx}{\linewidth}{lccccc} % 将表格宽度设置为当前行宽的80%
\toprule
& \multicolumn{1}{c}{Top-1} & \multicolumn{1}{c}{Top-5} & \multicolumn{1}{c}{Top-10} & \multicolumn{1}{c}{Top-20} & \multicolumn{1}{c}{Top-100} \\
\midrule
Random & 0.05 & 0.27 & 1.42 & 2.94 & 12.49 \\
SM & 5.87 & 14.65 & 22.37 & 28.24 & 43.66 \\
CE & 37.83 & 63.84 & 73.89 & 82.14 & \textbf{94.44} \\
BE & 29.17 & 51.95 & 60.67 & 72.12 & 89.62 \\
\retriever & \textbf{38.77} & \textbf{66.04} & \textbf{75.00} & \textbf{83.47} & 93.51 \\
\bottomrule
\end{tabularx}
\caption{Comparison between retrieval methods. SM, CE, BE stands for \textbf{S}tring \textbf{M}atch, \textbf{C}ross-\textbf{E}ncoder and \textbf{B}i-\textbf{E}ncoder respectively.}
\label{tab:retriever-main-results}
\end{table}

==> tables/table_representation_ablation_study.tex <==
\begin{table}[htbp]
%\small % 调整表格字体大小
\scriptsize
\begin{tabularx}{\linewidth}{lccccc} % 将表格宽度设置为当前行宽的80%
\toprule
& \multicolumn{1}{c}{Top-1} & \multicolumn{1}{c}{Top-5} & \multicolumn{1}{c}{Top-10} & \multicolumn{1}{c}{Top-20} & \multicolumn{1}{c}{Top-100} \\
\midrule
Full Table & 24.05 & 48.67 & 59.89 & 71.89 & 89.13 \\
No Table & 25.81 & 49.89 & 61.13 & 71.75 & 88.91 \\
Grounded Table & 29.17 & \textbf{} & 73.89 & 82.14 & \textbf{94.44} \\
\bottomrule
\end{tabularx}
\caption{Ablation Study on Table Representation with Bi-Encoder as the retriever.}
\label{tab:retriever-ablation-study}
\end{table}
